Broadcast Function Computation with Complementary Side Information

We consider the function computation problem in a three node network with one encoder and two decoders. The encoder has access to two correlated sources $X$ and $Y$. The encoder encodes $X^n$ and $Y^n$ into a message which is given to two decoders. Decoder 1 and decoder 2 have access to $X$ and $Y$ respectively, and they want to compute two functions $f(X,Y)$ and $g(X,Y)$ respectively using the encoded message and their respective side information. We want to find the optimum (minimum) encoding rate under the zero error and $\epsilon$-error (i.e. vanishing error) criteria. For the special case of this problem with $f(X,Y) = Y$ and $g(X,Y) = X$, we show that the $\epsilon$-error optimum rate is also achievable with zero error. This result extends to a more general `complementary delivery index coding' problem with arbitrary number of messages and decoders. For other functions, we show that the cut-set bound is achievable under $\epsilon$-error if $X$ and $Y$ are binary, or if the functions are from a special class of `compatible' functions which includes the case $f=g$.

==> Conclusion.tex <==
We first showed that for the complentary delivery problem,
the $\epsilon$-error rate is also achievable wih zero error. We further
showed that this is true for any complentary delivery index coding problem.
The optimal broadcast rate is established when either
For the function computation problem,  
the optimal broadcast rate is established when either
(i) $Z_1=Z_2$, (ii) $X,Y$ are binary random variables, or
(iii) $Z_1,Z_2$ are `compatible'. For the general case,
single letter inner and outer bounds are presented. 

% We provided a complete characterization of the rate region for the function computation
% problem in Gray-Wyner network. For Wyner network, a complete characterization is obtained
% when $Z_1=Z_2$ and a single letter outer bound is provided for the general case. 
% We further studied a broadcast function network which arises as a special case 
% of Wyner network. The optimal broadcast rate is established when either
% (i) $Z_1=Z_2$, (ii) $X,Y$ are binary random variables, or
% (iii) $Z_1,Z_2$ are `compatible'. For the general case,
% single letter inner and outer bounds are presented. 

